Disaster Resilience and Asset Prices

This paper investigates whether security markets price the effect of social distancing on firms' operations. We document that firms that are more resilient to social distancing significantly outperformed those with lower resilience during the COVID-19 outbreak, even after controlling for the standard risk factors. Similar cross-sectional return differentials already emerged before the COVID-19 crisis: the 2014-19 cumulative return differential between more and less resilient firms is of similar size as during the outbreak, suggesting growing awareness of pandemic risk well in advance of its materialization. Finally, we use stock option prices to infer the market's return expectations after the onset of the pandemic: even at a two-year horizon, stocks of more pandemic-resilient firms are expected to yield significantly lower returns than less resilient ones, reflecting their lower exposure to disaster risk. Hence, going forward, markets appear to price exposure to a new risk factor, namely, pandemic risk.

==> tables/table_returnregressions---replaceTRFDNAwith1_US_DN3_teleworkable_manual_wage_high50_low50_vw_fever_2020q1.tex <==
\begin{tabular}{L{5cm}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}} \toprule   &  \multicolumn{1}{C{1.4cm}}{ ret }  &   \multicolumn{1}{C{1.4cm}}{ capm }  &   \multicolumn{1}{C{1.4cm}}{ ff3 }  &   \multicolumn{1}{C{1.4cm}}{ ff4 }  &   \multicolumn{1}{C{1.4cm}}{ ff5 }  &   \multicolumn{1}{C{1.4cm}}{ ff6 }  \\ 
\midrule High resilience  &  -1.65^{***}  &  0.22^{*}  &  0.08  &  0.07  &  0.08  &  0.10  \\ 
%  &  \multicolumn{ 1}{c}{(0.44)}  &  \multicolumn{ 1}{c}{(0.12)}  &  \multicolumn{ 1}{c}{(0.13)}  &  \multicolumn{ 1}{c}{(0.13)}  &  \multicolumn{ 1}{c}{(0.08)}  &  \multicolumn{ 1}{c}{(0.08)}  \\ 
  &  \multicolumn{ 1}{c}{[-3.74]}  &  \multicolumn{ 1}{c}{[1.87]}  &  \multicolumn{ 1}{c}{[0.61]}  &  \multicolumn{ 1}{c}{[0.55]}  &  \multicolumn{ 1}{c}{[1.06]}  &  \multicolumn{ 1}{c}{[1.19]}  \\ 
Low resilience  &  -1.70^{***}  &  -0.30^{*}  &  -0.32^{*}  &  -0.23  &  -0.32^{**}  &  -0.27^{*}  \\ 
%  &  \multicolumn{ 1}{c}{(0.50)}  &  \multicolumn{ 1}{c}{(0.17)}  &  \multicolumn{ 1}{c}{(0.17)}  &  \multicolumn{ 1}{c}{(0.16)}  &  \multicolumn{ 1}{c}{(0.16)}  &  \multicolumn{ 1}{c}{(0.15)}  \\ 
  &  \multicolumn{ 1}{c}{[-3.39]}  &  \multicolumn{ 1}{c}{[-1.72]}  &  \multicolumn{ 1}{c}{[-1.85]}  &  \multicolumn{ 1}{c}{[-1.39]}  &  \multicolumn{ 1}{c}{[-2.08]}  &  \multicolumn{ 1}{c}{[-1.81]}  \\ 
\midrule High-minus-Low  &  0.05  &  0.52^{*}  &  0.40  &  0.29  &  0.40^{*}  &  0.37^{*}  \\ 
%  &  \multicolumn{ 1}{c}{(0.18)}  &  \multicolumn{ 1}{c}{(0.27)}  &  \multicolumn{ 1}{c}{(0.28)}  &  \multicolumn{ 1}{c}{(0.30)}  &  \multicolumn{ 1}{c}{(0.21)}  &  \multicolumn{ 1}{c}{(0.21)}  \\ 
  &  \multicolumn{ 1}{c}{[0.28]}  &  \multicolumn{ 1}{c}{[1.96]}  &  \multicolumn{ 1}{c}{[1.40]}  &  \multicolumn{ 1}{c}{[0.97]}  &  \multicolumn{ 1}{c}{[1.91]}  &  \multicolumn{ 1}{c}{[1.77]}  \\  \bottomrule \end{tabular}


==> tables/table_returnregressions---replaceTRFDNAwith1_US_HLR_dur_workplace_high50_low50_vw_fever_2020q1.tex <==
\begin{tabular}{L{5cm}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}} \toprule   &  \multicolumn{1}{C{1.4cm}}{ ret }  &   \multicolumn{1}{C{1.4cm}}{ capm }  &   \multicolumn{1}{C{1.4cm}}{ ff3 }  &   \multicolumn{1}{C{1.4cm}}{ ff4 }  &   \multicolumn{1}{C{1.4cm}}{ ff5 }  &   \multicolumn{1}{C{1.4cm}}{ ff6 }  \\ 
\midrule High resilience  &  -1.50^{***}  &  0.30^{***}  &  -0.00  &  0.02  &  -0.00  &  0.04  \\ 
%  &  \multicolumn{ 1}{c}{(0.45)}  &  \multicolumn{ 1}{c}{(0.05)}  &  \multicolumn{ 1}{c}{(0.07)}  &  \multicolumn{ 1}{c}{(0.07)}  &  \multicolumn{ 1}{c}{(0.05)}  &  \multicolumn{ 1}{c}{(0.05)}  \\ 
  &  \multicolumn{ 1}{c}{[-3.33]}  &  \multicolumn{ 1}{c}{[6.18]}  &  \multicolumn{ 1}{c}{[-0.04]}  &  \multicolumn{ 1}{c}{[0.27]}  &  \multicolumn{ 1}{c}{[-0.03]}  &  \multicolumn{ 1}{c}{[0.69]}  \\ 
Low resilience  &  -2.01^{***}  &  -0.41^{***}  &  -0.22^{**}  &  -0.24^{**}  &  -0.23^{*}  &  -0.26^{**}  \\ 
%  &  \multicolumn{ 1}{c}{(0.50)}  &  \multicolumn{ 1}{c}{(0.11)}  &  \multicolumn{ 1}{c}{(0.11)}  &  \multicolumn{ 1}{c}{(0.11)}  &  \multicolumn{ 1}{c}{(0.12)}  &  \multicolumn{ 1}{c}{(0.13)}  \\ 
  &  \multicolumn{ 1}{c}{[-4.02]}  &  \multicolumn{ 1}{c}{[-3.66]}  &  \multicolumn{ 1}{c}{[-2.11]}  &  \multicolumn{ 1}{c}{[-2.19]}  &  \multicolumn{ 1}{c}{[-1.85]}  &  \multicolumn{ 1}{c}{[-2.00]}  \\ 
\midrule High-minus-Low  &  0.52^{***}  &  0.70^{***}  &  0.22  &  0.26^{*}  &  0.22  &  0.29^{*}  \\ 
%  &  \multicolumn{ 1}{c}{(0.08)}  &  \multicolumn{ 1}{c}{(0.13)}  &  \multicolumn{ 1}{c}{(0.14)}  &  \multicolumn{ 1}{c}{(0.15)}  &  \multicolumn{ 1}{c}{(0.15)}  &  \multicolumn{ 1}{c}{(0.16)}  \\ 
  &  \multicolumn{ 1}{c}{[6.65]}  &  \multicolumn{ 1}{c}{[5.41]}  &  \multicolumn{ 1}{c}{[1.55]}  &  \multicolumn{ 1}{c}{[1.74]}  &  \multicolumn{ 1}{c}{[1.51]}  &  \multicolumn{ 1}{c}{[1.82]}  \\  \bottomrule \end{tabular}


==> tables/table_returnregressions---replaceTRFDNAwith1_US_KP_affected_share_high50_low50_vw_fever_2020q1.tex <==
\begin{tabular}{L{5cm}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}d{2.2}} \toprule   &  \multicolumn{1}{C{1.4cm}}{ ret }  &   \multicolumn{1}{C{1.4cm}}{ capm }  &   \multicolumn{1}{C{1.4cm}}{ ff3 }  &   \multicolumn{1}{C{1.4cm}}{ ff4 }  &   \multicolumn{1}{C{1.4cm}}{ ff5 }  &   \multicolumn{1}{C{1.4cm}}{ ff6 }  \\ 
\midrule High resilience  &  -1.48^{***}  &  0.46^{***}  &  0.23^{***}  &  0.16^{**}  &  0.23^{***}  &  0.17^{**}  \\ 
%  &  \multicolumn{ 1}{c}{(0.49)}  &  \multicolumn{ 1}{c}{(0.07)}  &  \multicolumn{ 1}{c}{(0.08)}  &  \multicolumn{ 1}{c}{(0.08)}  &  \multicolumn{ 1}{c}{(0.08)}  &  \multicolumn{ 1}{c}{(0.07)}  \\ 
  &  \multicolumn{ 1}{c}{[-3.02]}  &  \multicolumn{ 1}{c}{[6.59]}  &  \multicolumn{ 1}{c}{[2.69]}  &  \multicolumn{ 1}{c}{[2.06]}  &  \multicolumn{ 1}{c}{[3.04]}  &  \multicolumn{ 1}{c}{[2.28]}  \\ 
Low resilience  &  -1.76^{***}  &  -0.44^{***}  &  -0.43^{**}  &  -0.31^{**}  &  -0.44^{***}  &  -0.33^{**}  \\ 
%  &  \multicolumn{ 1}{c}{(0.47)}  &  \multicolumn{ 1}{c}{(0.16)}  &  \multicolumn{ 1}{c}{(0.17)}  &  \multicolumn{ 1}{c}{(0.15)}  &  \multicolumn{ 1}{c}{(0.17)}  &  \multicolumn{ 1}{c}{(0.15)}  \\ 
  &  \multicolumn{ 1}{c}{[-3.71]}  &  \multicolumn{ 1}{c}{[-2.71]}  &  \multicolumn{ 1}{c}{[-2.49]}  &  \multicolumn{ 1}{c}{[-1.99]}  &  \multicolumn{ 1}{c}{[-2.58]}  &  \multicolumn{ 1}{c}{[-2.14]}  \\ 
\midrule High-minus-Low  &  0.28^{***}  &  0.91^{***}  &  0.66^{***}  &  0.47^{**}  &  0.68^{***}  &  0.50^{**}  \\ 
%  &  \multicolumn{ 1}{c}{(0.10)}  &  \multicolumn{ 1}{c}{(0.22)}  &  \multicolumn{ 1}{c}{(0.25)}  &  \multicolumn{ 1}{c}{(0.22)}  &  \multicolumn{ 1}{c}{(0.24)}  &  \multicolumn{ 1}{c}{(0.21)}  \\ 
  &  \multicolumn{ 1}{c}{[2.84]}  &  \multicolumn{ 1}{c}{[4.09]}  &  \multicolumn{ 1}{c}{[2.65]}  &  \multicolumn{ 1}{c}{[2.15]}  &  \multicolumn{ 1}{c}{[2.87]}  &  \multicolumn{ 1}{c}{[2.40]}  \\  \bottomrule \end{tabular}

